Classification of Gapped Domain Walls of Topological Orders in 2+1 dimensions: A Levin-Wen Model Realization

This paper introduces a novel systematic construction of gapped domain walls (GDWs) within the Levin-Wen (LW) model. By gluing two LW models along their open sides in a compatible way, we achieve a complete GDW classification by subsets of bulk input data, which encompass the classifications in terms of bimodule categories. A generalized bimodule structure is introduced to capture domain-wall excitations. Furthermore, we demonstrate that folding along any GDW yields a gapped boundary (GB) described by a Frobenius algebra of the input UFC for the folded model, thus bridging our GDW classification and the GB classification in \cite{hu2018boundary}.

==> images/e-m_exchange/eq__basis-multiplication_1.tex <==
\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        
\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1, baseline=(XXXX.south) ]
\path (0,57);\path (75.31640625,0);\draw    ($(current bounding box.center)+(0,0.3em)$) node [anchor=south] (XXXX) {};
%Straight Lines [id:da4018866490161268] 
\draw [color={rgb, 255:red, 33; green, 55; blue, 191 }  ,draw opacity=1 ][line width=0.75]    (56.75,52.52) -- (34.71,30.48) ;
\draw [shift={(47.78,43.55)}, rotate = 225] [fill={rgb, 255:red, 33; green, 55; blue, 191 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- (3.56,0) -- cycle    ;
%Straight Lines [id:da6408485731167761] 
\draw [color={rgb, 255:red, 33; green, 55; blue, 191 }  ,draw opacity=1 ][line width=0.75]    (12.74,52.45) -- (34.71,30.48) ;
\draw [shift={(21.67,43.52)}, rotate = 315] [fill={rgb, 255:red, 33; green, 55; blue, 191 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- (3.56,0) -- cycle    ;
%Straight Lines [id:da127031431726077] 
\draw [color={rgb, 255:red, 33; green, 55; blue, 191 }  ,draw opacity=1 ][line width=0.75]    (34.71,3.71) -- (34.71,30.48) ;
\draw [shift={(34.71,14.19)}, rotate = 90] [fill={rgb, 255:red, 33; green, 55; blue, 191 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- (3.56,0) -- cycle    ;
%Shape: Circle [id:dp8022541365311111] 
\draw  [color={rgb, 255:red, 33; green, 55; blue, 191 }  ,draw opacity=1 ][fill={rgb, 255:red, 33; green, 55; blue, 191 }  ,fill opacity=1 ] (31.75,30.48) .. controls (31.75,28.85) and (33.08,27.53) .. (34.71,27.53) .. controls (36.34,27.53) and (37.67,28.85) .. (37.67,30.48) .. controls (37.67,32.12) and (36.34,33.44) .. (34.71,33.44) .. controls (33.08,33.44) and (31.75,32.12) .. (31.75,30.48) -- cycle ;
% Text Node
\draw (-0.5,33.2) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize]  {$M_{k}$};
% Text Node
\draw (48.82,32.99) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize]  {$M_{j}$};
% Text Node
\draw (36.71,5.41) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize]  {$M_{i}$};
% Text Node
\draw (20.5,20.2) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize]  {$v$};
\end{tikzpicture}

